COPAL-ID: Indonesian Language Reasoning with Local Culture and Nuances

We present COPAL-ID, a novel, public Indonesian language common sense reasoning dataset. Unlike the previous Indonesian COPA dataset (XCOPA-ID), COPAL-ID incorporates Indonesian local and cultural nuances, and therefore, provides a more natural portrayal of day-to-day causal reasoning within the Indonesian cultural sphere. Professionally written by natives from scratch, COPAL-ID is more fluent and free from awkward phrases, unlike the translated XCOPA-ID. In addition, we present COPAL-ID in both standard Indonesian and in Jakartan Indonesian-a dialect commonly used in daily conversation. COPAL-ID poses a greater challenge for existing open-sourced and closed state-of-the-art multilingual language models, yet is trivially easy for humans. Our findings suggest that general multilingual models struggle to perform well, achieving 66.91% accuracy on COPAL-ID. South-East Asian-specific models achieve slightly better performance of 73.88% accuracy. Yet, this number still falls short of near-perfect human performance. This shows that these language models are still way behind in comprehending the local nuances of Indonesian.

==> tables/analysis_category.tex <==
\begin{table*}[]
\centering
\small
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Standard}} & \multicolumn{3}{c}{\textbf{Colloquial}}   \\  
\cmidrule{2-7}
& \textbf{Culture} & \textbf{Language} & \textbf{Terminology} & \textbf{Culture} & \textbf{Language} & \textbf{Terminology}  \\
\midrule
{\textbf{Finetuned}} & & & & & & \\
\hspace{6pt}XLMR-Large      & 61.70 & 71.96 & 64.58   &  59.93 & 71.03 & 63.76 \\
\hspace{6pt}XLMR-Base & 55.32 & 63.55 & 55.31 & 57.45 & 60.75 & 58.04      \\
\midrule
{\textbf{Open prompting}}   \\
\hspace{6pt}BLOOMZ-7B & 61.35 & 72.90 & 64.03 & 56.03 & 58.88 & 61.04    \\ 
\hspace{6pt}PolyLM 13B & 59.22 & 70.09 & 62.67 & 55.32 & 63.55 & 56.40 \\

\midrule
{\textbf{Closed prompting}}                                                                \\
\hspace{6pt}ChatGPT & 75.53 & 81.31 & 76.57 & 71.63 & 77.57 & 75.20         \\

\hspace{6pt}GPT-4 & 87.23 & 96.26 & 87.74 & 89.36 & 88.79 & 90.46  \\ 
\midrule
\hspace{6pt} Human (Average) & 93.97 & 97.66 & 94.28 & 94.68 & 98.13 & 95.78     \\ 
\bottomrule

\end{tabular}
\caption{Accuracy Models on the benchmark per category}
\label{analogy}
\end{table*}

==> tables/crosslingual.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering

\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Accuracy}}                                                \\  
                                & \textbf{Monolingual} & \textbf{Translate-test} & \textbf{Crosslingual}  \\ 
                                \midrule
{\textbf{Finetuned models}} \\
\hspace{8pt}XLMR-Large            &  64.22 &  52.06  &  53.67  \\
\hspace{8pt}XLMR-Base           &  55.99 &  52.24  &  52.95   \\
\midrule
{\textbf{Open models prompting}}                                                                \\
\hspace{8pt}BLOOMZ 7B &  65.47  &  55.81  &  62.97    \\
\hspace{8pt}PolyLM 13B &  62.79  &  55.99  &  63.33      \\
\bottomrule

\end{tabular}
\caption{Comparison of accuracy on different translation scenarios.}
\label{lingual}
\end{table*}

==> tables/data_creation.tex <==
\begin{table*}[bp]
\footnotesize
\centering
\begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.05\linewidth}p{0.22\linewidth}@{}}
\toprule
Premise & Correct Option & Incorrect Option & Verdict & Note  \\ 

\midrule

    Ia ingin memberbaharui SIM-C miliknya 
    & Ia datang ke kantor polisi
    & Ia datang ke toko ponsel
    & U
    & \multirow{4}{\linewidth}{\textbf{Correctness}. We need to go to SAMSAT (not the police station) to obtain SIM-C (a driving license)} \\
 \textit{(He/she wants to renew his/her SIM-C)} & \textit{(He/she goes to police station)} & \textit{(He/she goes to phone shop)} & & \\

\midrule

    Hari ini ada gangguan sinyal 
    & Perjalanan kereta terlambat
    & Perjalanan pesawat terlambat
    & R
    & \multirow{2}{\linewidth}{\textbf{Appropriateness}. Signalling failures are not uniquely cultural to Indonesia.} \\
 \textit{(Today there is a signalling failure)} & \textit{(Trains are delayed)} & \textit{(Flights are delayed)} & & \\

\midrule

    Dia hendak beribadah pada hari Minggu
    & Dia pergi ke gereja
    & Dia pergi ke wihara
    & R
    & \multirow{2}{\linewidth}{\textbf{Ambiguity}. Churches and Viharas both provide religious services on Sundays.} \\
 \textit{(He/she is going to pray on Sunday)} & \textit{(He/she goes to the church)} & \textit{(He/she goes to the vihara)} & & \\

\midrule

    Saat lebaran, suasana kota Jakarta sangat sepi
    & Masyarakatnya sedang pulang kampung
    & Ada pawai di Jakarta
    & R
    & \multirow{2}{\linewidth}{\textbf{Difficulty}. Parade is never quiet, making this data too easy.} \\
 \textit{(During Eid, Jakarta becomes quiet.)} & \textit{(The citizens are going to their hometown)} & \textit{(There is a parade in Jakarta)} & & \\	

\midrule

    Ayah tidak kunjung tiba karena pesawatnya terlambat berjam-jam
    & Ayah naik <Maskapai A>
    & Ayah naik <Maskapai B>)
    & R
    & \multirow{2}{\linewidth}{\textbf{Ethics}. The original data directly mentions certain airline brands, perpetuating certain stereotypes about them.} \\
 \textit{(Father has not arrived yet because his airline is delayed for hours)} & \textit{(Father flies with <Airline A>)} & \textit{(Father flies with <Airline B>)} & & \\	

\midrule

    Anak itu ketakutan
    & Ia mimpi melihat pocong
    & Ia mimpi melihat porli
    & U
    & \multirow{3}{\linewidth}{\textbf{Clarity}. Pocong is a local ghost, while porli is a typo of Polri (abbreviation of Indonesian national police)} \\
 \textit{(That child is terrified)} & \textit{(He/she dreams of pocong)} & \textit{(He/she dreams of porli)} & & \\
 & {} \\ 


\bottomrule
\end{tabular}
\vspace{-0.2cm}
\caption{
Candidate of \dataname examples from the first iteration that are rejected or need revision. U means ``needs small update/rephrase'', while R means rejected and needs to be replaced with new data.
}
\label{tab:example_data_cross_review}
\end{table*}

\begin{table*}[bp]
\footnotesize
\centering

\vspace{0.5cm}

\begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.05\linewidth}p{0.22\linewidth}@{}}
\toprule
Premise & Correct Option & Incorrect Option & Verdict & Note  \\ 

\midrule

    Saya mau berangkat sekolah
    & Saya mencium tangan orang tua
    & Saya menunggu bis sekolah
    & A
    & \multirow{4}{\linewidth}{These two data have the same topic of 'kissing parent's hand' and both phrasings are almost identical to each other. In this case, we only accept one of them.} \\
 \textit{(I am going to school)} & \textit{(I kiss my parent's hand)} & \textit{(I wait for the school bus)} & \\
 Anak itu akan berangkat sekolah & Anak itu cium tangan orang tuanya & Anak itu cium dahi orang tuanya & R &  \\ 
 \textit{(That child is going to school)} & \textit{(That child kisses his/her parent's hand)} & \textit{(That child kisses his/her parent's forehead)} & \\ 

\midrule

    Ada kasus demam berdarah di komplek itu
    & Mereka mengadakan penyemprotan
    & Mereka memanggil detektif
    & A
    & \multirow{4}{\linewidth}{Although these two data mention the same topic of ``dengue fever'', the context on how the topic is used is quite different. Thus, we accept both data.} \\
 \textit{(There's a dengue fever case in that area)} & \textit{(They spray the area)} & \textit{(They call a detective)} & \\
 Di musim penghujan, kampungku mengadakan fogging & Pemerintah ingin membasmi demam berdarah & Pemerintah ingin membasmi malaria & A &  \\ 
 \textit{(In rainy season, my village conducts a fogging)} & \textit{(The government wants to prevent dengue fever)} & \textit{(The government wants to prevent malaria)} & \\ 

\bottomrule

\end{tabular}
\caption{
Candidate of \dataname examples that are marked as duplicate or similar to each other. A means accepted, R means rejected and needs to be replaced with new data. }
\label{tab:example_data_duplicate}
\end{table*}

==> tables/maintable-old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering

\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Accuracy}}                                                \\  
                                & \textbf{XCOPA-ID} & \textbf{\dataname} & \textbf{\dataname}  & \textbf{\dataname} \\ 
& & (standard) & (colloquial) & (translated) \\
                                \midrule
{\textbf{Finetuned models}}                                                                         \\
\hspace{8pt}XLMR-Base            &  66.80  &  55.99  &  57.42     &  52.24\\
\hspace{8pt}XLMR-Large           &  79.40  &  64.22  &  62.97     &  52.06  \\
\hspace{8pt}mBERT                &  59.60  &  55.64  &  56.35     &  56.53  \\
\hspace{8pt}IndoBERT             &  67.60  &  61.00  &  60.64    &  - \\
\midrule
{\textbf{Open models prompting}}                                                                \\
\hspace{8pt}BLOOMZ-7B (5-shot)            &  76.20  &  65.54  &  59.64     &  56.07  \\
\hspace{8pt}Bactrian-X (5-shot)   &  71.20  &  62.14  &  58.04      &  55.00   \\
\hspace{8pt}LLaMA2 7B (5-shot)    &  64.20  &  58.04  &  54.29      &  55.36  \\
% LLaMA2-chat 7B (5-shot)         &                   &                    &                                            \\
\hspace{8pt}PolyLM 13B (5-shot)   &  71.20  &  62.86  &  58.39      & 56.07  \\
\midrule
{\textbf{Closed models prompting}}                                                                \\
\hspace{8pt}ChatGPT (5-shot)      &  90.80  &  77.28  &  74.24  &  -   \\
\hspace{8pt}GPT-4 (5-shot)        &  97.20  &  89.09  &  89.62  &  -  \\ \midrule
\textbf{Human}      &  -  &  95.00  &  95.62  &  -    \\
\bottomrule

\end{tabular}
\caption{Comparison of accuracy of finetuned, prompting with open, and prompting with closed models. For finetuned model, we train and validate on Indonesian dataset GEN-X except for \dataname- translated in which we use COPA-EN.
For IndoBERT, we did not train on COPA-EN as it is an Indonesian model only. The prompt results are the maximum among different attempted prompts.}
\label{main-exp}
\end{table*}
